Bootstrapping Semantic Segmentation with Regional Contrast

We present ReCo, a contrastive learning framework designed at a regional level to assist learning in semantic segmentation. ReCo performs semi-supervised or supervised pixel-level contrastive learning on a sparse set of hard negative pixels, with minimal additional memory footprint. ReCo is easy to implement, being built on top of off-the-shelf segmentation networks, and consistently improves performance in both semi-supervised and supervised semantic segmentation methods, achieving smoother segmentation boundaries and faster convergence. The strongest effect is in semi-supervised learning with very few labels. With ReCo, we achieve high-quality semantic segmentation models, requiring only 5 examples of each semantic class. Code is available at https://github.com/lorenmt/reco.

==> image/sampling.tex <==
\begin{tikzpicture}

\definecolor{color3}{RGB}{173, 180, 190}
\definecolor{color2}{RGB}{111, 176, 216}
\definecolor{color1}{RGB}{37, 90, 169}

\begin{axis}[
every axis y label/.style={at={(current axis.north west)},above=1mm},
every x tick label/.append style={font=\footnotesize},
width=8cm, height=4.5cm,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.4, xmax=3.4,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={\makecell[l]{Random Query \\Random Key}, \makecell[l]{Active Query \\Random Key}, \makecell[l]{Easy Query \\Active Key}, {\normalsize Ours}},
y grid style={white!69.0196078431373!black},
ylabel={mIoU},
ymin=44, ymax=51,
ytick={44, 46, 48, 50},
ytick style={color=black}
]
\draw[draw=none,fill=color2] (axis cs:-0.325,0) rectangle (axis cs:0.325,46.56);
\draw[draw=none,fill=color2] (axis cs:0.675,0) rectangle (axis cs:1.325,46.38);
\draw[draw=none,fill=color2] (axis cs:1.675,0) rectangle (axis cs:2.325,45.81);
\draw[draw=none,fill=color1] (axis cs:2.675,0) rectangle (axis cs:3.325,49.83);
\draw[draw=none,fill=color3] (axis cs:-0.325,0) rectangle (axis cs:0.325,45.61);
\draw[draw=none,fill=color3] (axis cs:0.675,0) rectangle (axis cs:1.325,45.61);
\draw[draw=none,fill=color3] (axis cs:1.675,0) rectangle (axis cs:2.325,45.61);
\draw[draw=none,fill=color3] (axis cs:2.675,0) rectangle (axis cs:3.325,45.61);
\node[above] at (0, 46.56) {\footnotesize 46.56};
\node[above] at (1, 46.38) {\footnotesize 46.38};
\node[above] at (2, 45.81) {\footnotesize 45.81};
\node[above] at (3, 49.83) {\footnotesize 49.83};
\end{axis}


\end{tikzpicture}

